On the Robustness of Arabic Speech Dialect Identification

Arabic dialect identification (ADI) tools are an important part of the large-scale data collection pipelines necessary for training speech recognition models. As these pipelines require application of ADI tools to potentially out-of-domain data, we aim to investigate how vulnerable the tools may be to this domain shift. With self-supervised learning (SSL) models as a starting point, we evaluate transfer learning and direct classification from SSL features. We undertake our evaluation under rich conditions, with a goal to develop ADI systems from pretrained models and ultimately evaluate performance on newly collected data. In order to understand what factors contribute to model decisions, we carry out a careful human study of a subset of our data. Our analysis confirms that domain shift is a major challenge for ADI models. We also find that while self-training does alleviate this challenges, it may be insufficient for realistic conditions.

==> tables/msa_vs_da_results.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{lcc} \hline 
  & \multicolumn{2}{c}{\textbf{MSA vs DA evaluation}} \\
                 &  \textbf{ACC}  & \textbf{F\textsubscript{1}} \\
                 \hline Majority Class  & -  & -
 \\
  HuBERT Fixed  & - & - \\
 HuBERT(MSAvsDA)  & -  &  - \\
 HuBERT(ADI18)  & - & - \\  
 HuBERT(Self-trained)  & - & - \\ \hline 

\end{tabular}
\caption[-]{-}
\label{tab:msavsda}
\end{table}
